Scene-aware Generative Network for Human Motion Synthesis

We revisit human motion synthesis, a task useful in various real world applications, in this paper. Whereas a number of methods have been developed previously for this task, they are often limited in two aspects: focusing on the poses while leaving the location movement behind, and ignoring the impact of the environment on the human motion. In this paper, we propose a new framework, with the interaction between the scene and the human motion taken into account. Considering the uncertainty of human motion, we formulate this task as a generative task, whose objective is to generate plausible human motion conditioned on both the scene and the human initial position. This framework factorizes the distribution of human motions into a distribution of movement trajectories conditioned on scenes and that of body pose dynamics conditioned on both scenes and trajectories. We further derive a GAN based learning approach, with discriminators to enforce the compatibility between the human motion and the contextual scene as well as the 3D to 2D projection constraints. We assess the effectiveness of the proposed method on two challenging datasets, which cover both synthetic and real world environments.

==> Sections/section_introduction.tex <==
\section{Introduction}
\label{sec:intro}

%
The ability of synthesizing human motions is beneficial for many real-world applications, 
including virtual reality, computer games, accident prevention and human behavior understanding.
%
While previous methods~\cite{fragkiadaki2015recurrent, martinez2017human, li2017auto, yan2019convolutional, chuan2020action2motion, cai2018deep, barsoum2018hp, yang2018pose} for human motion synthesis often focus only on the movements of human bodies, the influence of scene context is neglected.
%
However, scene context plays an essential role in human motions.
%
At first, the concept of human motion actually consists of two parts,
namely body movements, and the trajectory of human in the surrounding scene.
%
There are infinite ways for a person to move from one place to another with identical body movements, and they are all valid human motions.
%
Therefore leaving trajectories in the scene aside will significantly decrease diversity of synthesized human motions.
%
Moreover, scene context also provides strong semantic guidances for human motions,
as most of our actions are closely related to objects in the scene (\eg~sitting on a chair),
and we should avoid colliding with any objects or walls in the scene.

%
Inspired by the importance of scene context, in this paper we aim at synthesizing human motions with scene context as the guidance, which is a newly emerged topic with few early attempts~\cite{cao2020long}.
%
Following~\cite{cao2020long}, we represent scene context using a RGB image,
which are relatively easy to acquire in real scenarios.
%
There are two major challenges to handle when involving scene context.
%
The first challenge is how to model the joint distribution of trajectories in the scene and movements of the body, so that the diversity of human motions can be fully captured.
%
The other challenge is how to effectively reflect the semantic guidance provided by the scene context.
%
Specifically, to avoid collision we need to know the geometric configuration of the scene context (\eg~where the wall is), which is naturally a 3D concept, and we can only infer it from a 2D image and a depth map.
%
An effective design is thus needed. 
%
In the meantime, such a design should also be efficient, otherwise it may bring too much overhead to the synthesis process.

\begin{figure}[t]
\footnotesize
\centering
\renewcommand{\tabcolsep}{1pt} % adjust horizontal space
%\ra{1} % adjust vertical space
\begin{center}
\begin{tabular}{ccc}
\includegraphics[width=0.3\linewidth]{Sections/Figures/t-1-1.jpg} &
\includegraphics[width=0.3\linewidth]{Sections/Figures/t-1-2.jpg} &
\includegraphics[width=0.3\linewidth]{Sections/Figures/t-1-3.jpg} \\
\includegraphics[width=0.3\linewidth]{Sections/Figures/t-2-1.jpg} &
\includegraphics[width=0.3\linewidth]{Sections/Figures/t-2-2.jpg} &
\includegraphics[width=0.3\linewidth]{Sections/Figures/t-2-3.jpg} \\
(a) &
(b) &
(c)

\end{tabular}
\end{center}
\caption{\textbf{Visualtion results of the sampled human motions from our method in different scenes}.
Our method not only can synthesize human motions which go to different goals in the scene, such as the human motions shown in (a) and (c), but also can syntheisze human motions walk to the same goal with different trajectories, such as (b) and (c).}
\label{fig:teaser}
\end{figure}

%
We propose a scene-aware fully generative framework to tackle these challenges introduced by the scene context.
%
Specifically, we divide the joint distribution of trajectories in the scene and body movements into two distributions, namely the distribution of trajectories and the conditional distribution of body movements given a trajectory.
%
Inspired the success of convolutional sequence generation networks (CSGN) in skeleton-based action synthesis \cite{yan2019convolutional}, a CSGN is used to model the body movements in the form of skeleton sequences, taking a trajectory in the scene as input.
%
As for the distribution of trajectories, while Cao~\etal~\cite{cao2020long} treat it as the distribution of end points, and use a \emph{deterministic} function to generate the trajectory given a pair of start and end points, we argue that such a treatment may lead to gaps between the learned distribution and the actual one since there could be infinite ways even if both the start and the end points are fixed, as shown in Fig~\ref{fig:teaser}.
%
In contrast, we utilize another CSGN to directly model trajectories as in body movements modeling, without making any assumptions. 
%
In this way our framework is fully generative, and is capable of capturing the diversity of human motions in different levels.
%

To fulfill the geometric comaptiblity, it is crucial to introduce the geometry structure of the scene as prior knowledge into our synthesis framework.
%
Therefore, we supervise the encoder for extracting information of the scene by the depth map.
%
Under this supervision, this encoder can provide geometry-aware feature of the scene and we do not need to provide depth information of the scene during inference, which can be used more easily.
%\textcolor{red}{(bdai: you may need to expand this a bit. extract features sounds trivial)}
%
Moreover, we also propose a projection discriminator and a context discriminator to further encourage
the compatibility between synthesized human motions and the surrounding scene context.
%
We deploy the projection discriminator on the 2D human motion in image coordinate space from the 3D human motion, because the abnormal human motion in the scene can be clearly exhibited by the scale changes of human sequence in image coordinate space.
%
Therefore, this discriminator encourages the generator to synthesize trajectories following the global structure of scene.
%
Besides, the moving direct of human movement is also can be clearly defined in the 2D space by coordinate and human scale changes.
%
This discriminator also can encourage the compatibility between the trajectory and body movements.
%
To prevent the collusion of the synthesized human motions to the objects in the scene, we deploy this context discriminator to the relative depth sequence of the human motion to the local environment at each time step.
%
This discriminator encourages human move to the correct places surrounding to these objects.
 
%\textcolor{red}{(bdai: may need to refine the sentence to give a little bit details, "a projection discriminator and a context discriminator" sounds trivial)}

We choose two challenging datasets to evaluate the effectiveness of 
our proposed geometry-aware fully generative framework,
covering both a synthesized environment (\emph{GTA-IM}~\cite{cao2020long}) and a real environment (\emph{PROX}~\cite{PROX:2019}).
On both datasets,
the proposed framework is capable of synthesizing promising human motions,
in terms of the fidelity of each independent sequence,
the diversity of multiple sampled sequences,
as well as the consistency between synthesized sequences and their corresponding scenes.
To better quantitatively assess different methods,
we also propose a series of new metrics for human motion synthesis with scene context,
including Motion FID, which is inspired by FID for image synthesis,
and Collision Rate, which borrows insights from 3D computer games and examines the potential collisions between human motions and the scenes.

To summarize our contributions:
1) we reformulate the task of human motion synthesis with scene context to avoid limitations of the existing setting.
We further propose a series of quantitative metrics to enhance the evaluation protocol of this task.
2) We develop a novel geometry-aware fully generative framework for this task,
which explicitly takes the scene geometry into consideration and captures the diversity of human motions in a scene from multiple levels.
3) We propose two geometry-aware discriminators to encourage the compatibility between synthesized human motions and their corresponding scenes.


